Advanced Optimal Control Methods for Spin Systems

Work within this thesis advances optimal control algorithms for application to magnetic resonance systems. Specifically, presenting a quadratically convergent version of the gradient ascent pulse engineering method. The work is formulated in a superoperator representation of the Liouville-von Neumann equation. A Newton-grape method is developed using efficient calculation of analytical second directional derivatives. The method is developed to scale with the same complexity as methods that use only first directional derivatives. Algorithms to ensure a well-conditioned and positive definite matrix of second directional derivatives are used so the sufficient conditions of gradient-based numerical optimisation are met. A number of applications of optimal control in magnetic resonance are investigated: solid-state nuclear magnetic resonance, magnetisation-to-singlet pulses, and electron spin resonance experiments.

==> Chapter_1/min_tangents.tikz.tex <==
\begin{tikzpicture}[tight background]
\begin{groupplot}[
		group style={
		group name=my plots,
		group size=2 by 2,
		horizontal sep=2em,
		vertical sep=2em,
		},
    width=0.5\columnwidth,
    axis lines=middle,
    xmin=-2.95, xmax=2.95,
    ymin=-1.45, ymax=3.45,
    x label style={at={(ticklabel* cs:1.00)},anchor=west},
    xtick distance=1, 
    ytick distance=1,
    minor x tick num = 3,
    minor y tick num = 3,
    grid=both,
    xlabel=$x$,
    ylabel=$y$,
    x axis line style={latex-latex},
    y axis line style={latex-latex},
]
\nextgroupplot[title style={at={(0.5,1)},anchor=center,align=center},
	      title={\plotlabel{a} $^{}_{}${\scshape Extrema of $f(x)$. Roots of $f^{\prime}(x)$}$^{}_{}$},]
               \coordinate (top) at (rel axis cs:0,1);
\addplot+[smooth,MatlabBlue,mark=none,thick,samples=40] {1-x+(x^3)/3};
\addplot+[smooth,MatlabOrange,mark=none,thick,samples=40] {-1+x^2};
\addplot+[black,dashed,mark=none,thick] coordinates {(-1,0) (-1,5/3)};
\addplot+[black,dashed,mark=none,thick] coordinates {(1,0) (1,1/3)};

\nextgroupplot[title style={at={(0.5,1)},anchor=center,align=center},
	      title={\plotlabel{b} $^{}_{}${\scshape Tangent to $f^{\prime}(x)$: Iteration\#1}$^{}_{}$},]
\addplot+[smooth,MatlabOrange,mark=none,thick,samples=40] {-1+x^2};
\addplot+[MatlabOrange,mark=*] coordinates {(2,4-1)};
\addplot+[MatlabYellow,mark=none,thick] {4*x - 5};
\addplot+[MatlabYellow,mark=oplus] coordinates {(1.25,0)};

\nextgroupplot[title style={at={(0.5,1)},anchor=center,align=center},
	      title={\plotlabel{c} $^{}_{}${\scshape Tangent to $f^{\prime}(x)$: Iteration\#2}$^{}_{}$},]
\addplot+[smooth,MatlabOrange,mark=none,thick,samples=40] {-1+x^2};
\addplot+[MatlabOrange,mark=*] coordinates {(1.25,0.5625)};
\addplot+[MatlabYellow,mark=none,thick] {2.5*x - 2.5625};
\addplot+[MatlabYellow,mark=oplus] coordinates {(1.025,0)};

\nextgroupplot[title style={at={(0.5,1)},anchor=center,align=center},
	      title={\plotlabel{d} $^{}_{}${\scshape Tangents to $f(x)$}$^{}_{}$},]
\addplot+[smooth,MatlabBlue,mark=none,thick,samples=40] {1-x+((x^3)/3)};
\addplot+[MatlabMagenta,mark=none,thin] {(((2^2) -1)*(x-2)) + 5/3};
\addplot+[MatlabMagenta,mark=none,thin] {(((1.25^2) -1)*(x-1.25)) + 0.401041666666667};
\addplot+[MatlabMagenta,mark=none,thin] {((1.025^2) -1)*(x-1.025) + 0.333963541666667};
\addplot+[MatlabMagenta,mark=none,thin] {((1.000304878048780^2) -1)*(x-1.000304878048780) + 0.333333426293404};
\addplot+[MatlabMagenta,mark=none,thin] {((1.000000046461147^2) -1)*(x-1.000000046461147) + 0.333333333333335};
    
         \coordinate (bot) at (rel axis cs:1,0);
\end{groupplot}

\path[name path=p1] (top-|current bounding box.west)-- node[anchor=south,rotate=90] {} (bot-|current bounding box.west);
\path[name path=p2] (top|-current bounding box.south)-- coordinate(legendpos) (bot|-current bounding box.south);

\matrix[matrix of nodes, anchor=north, inner sep=0.2em, font=\sc\scriptsize,
    column 1/.style={anchor=base east},
    column 2/.style={anchor=base west},
    column 3/.style={anchor=base east},
    column 4/.style={anchor=base west}] at (legendpos)
  {\draw[legendline={MatlabBlue}{1}] (-0.25,0.1) -- (0.25,0.1); & $y=f(x)=\tfrac{1}{3}x^3-x+1$ & [0.1\columnwidth]
   \draw[legendline={MatlabMagenta}{1}] (-0.25,0.1) -- (0.25,0.1); & tangent to $f(x)$ \\
   \draw[legendline={MatlabOrange}{1}] (-0.25,0.1) -- (0.25,0.1); & $y=f^{\prime}(x)=x^2-1$ & [0.1\columnwidth]
   \draw[legendline={MatlabYellow}{1}] (-0.25,0.1) -- (0.25,0.1); & tangent to $f^{\prime}(x)$ \\};
\end{tikzpicture}

==> Chapter_1/robot_arm.tikz.tex <==
\newcommand{\nvar}[2]{%
    \newlength{#1}
    \setlength{#1}{#2}
}

% Define a few constants for drawing
\nvar{\dg}{0.3cm}
\def\dw{0.25}\def\dh{0.35}
% Define commands for links, joints and such
\def\link{\draw [double distance=1.5mm, very thick] (0,0)--}
\def\joint{%
    \filldraw [thick,fill=white] (0,0) circle (5pt) node {$T_1$};
}
\def\grip{%
    \draw[ultra thick](0cm,\dg)--(0cm,-\dg);
    \fill (0cm, 0.5\dg)+(0cm,1.5pt) -- +(0.6\dg,0cm) -- +(0pt,-1.5pt);
    \fill (0cm, -0.5\dg)+(0cm,1.5pt) -- +(0.6\dg,0cm) -- +(0pt,-1.5pt);
}

\def\robotbase{%
    \draw[thick,rounded corners=6pt] (-\dw,-\dh)-- (-\dw, 0) --
        (0,\dh)--(\dw,0)--(\dw,-\dh);
    \draw (-0.5,-\dh)-- (2.5,-\dh);
    \fill[pattern=north east lines] (-0.5,-0.5) rectangle (2.5,-\dh);
}

% This macro draws a three link manipulator.
% Input parameters:
%   #1 theta_1
%   #2 L_1
%   #3 theta_2
%   #4 L_2
%   #5 theta_3
%   #6 L_3
%
% Example:
%   \threelink{60}{2}{-70}{2}{30}{1}
\newcommand{\threelink}[6]{%
    \robotbase
    \link(#1:#2);
    \filldraw [thick,fill=white] (0,0) circle (5pt) node {\scriptsize\bf{A}};
    \begin{scope}[shift=(#1:#2), rotate=#1]
        \link(#3:#4);
        \filldraw [thick,fill=white] (0,0) circle (5pt) node {\scriptsize\bf{B}};
        \begin{scope}[shift=(#3:#4), rotate=#3]
            \link(#5:#6);
            \filldraw [thick,fill=white] (0,0) circle (5pt) node {\scriptsize\bf{C}};
            \begin{scope}[shift=(#5:#6), rotate=#5]
                \grip
            \end{scope}
        \end{scope}
    \end{scope}
}

\begin{tikzpicture}[tight background]
    \begin{scope}[name=scope1,xshift=-3cm]
        \threelink{90}{2}{-90}{2}{-90}{1}
    \end{scope}
    \draw [font=\footnotesize\scshape,align=center] (0,0) -- node [anchor=south] {Control$^{}_{}$} (2,0) node[inputarrow,rotate=0] {};
    \begin{scope}[xshift=3cm]
        \threelink{60}{2}{-60}{2}{0}{1}
    \end{scope}
    \begin{scope}[name=scope2,xshift=-4cm,yshift=-4cm]
        % Illustration of two different solutions to the inverse kinematic
        % problem.
        \begin{scope}[color=black!25]
            \threelink{90}{2}{-90}{2}{-90}{1}
        \end{scope}
	\threelink{60}{2}{-90}{2}{-90}{1}
    \end{scope}
    \begin{scope}[name=scope3,yshift=-4cm]
        % Illustration of two different solutions to the inverse kinematic
        % problem.
        \begin{scope}[color=black!25]
            \threelink{60}{2}{-90}{2}{-90}{1}
        \end{scope}
	\threelink{60}{2}{-60}{2}{-90}{1}
    \end{scope}
    \begin{scope}[name=scope4,yshift=-4cm,xshift=4cm]
        % Illustration of two different solutions to the inverse kinematic
        % problem.
        \begin{scope}[color=black!25]
            \threelink{60}{2}{-60}{2}{-90}{1}
        \end{scope}
	\threelink{60}{2}{-60}{2}{0}{1}
    \end{scope}
    \begin{scope}[name=scope5,yshift=-8cm,xshift=-2cm]
        % Illustration of two different solutions to the inverse kinematic
        % problem.
        \begin{scope}[color=black!25]
            \threelink{90}{2}{-90}{2}{-90}{1}
        \end{scope}
	\threelink{60}{2}{-60}{2}{-60}{1}
    \end{scope}
    \begin{scope}[name=scope6,yshift=-8cm,xshift=2cm]
        % Illustration of two different solutions to the inverse kinematic
        % problem.
        \begin{scope}[color=black!25]
            \threelink{60}{2}{-60}{2}{-60}{1}
        \end{scope}
	\threelink{60}{2}{-60}{2}{0}{1}
    \end{scope}
    \node [font=\scriptsize\scshape,text=black, at={(-2.5,2.4))}] {\circled{1} Initial state$^{}_{}$};
    \node [font=\scriptsize\scshape,color=white,text=black, at={(4.5,2.4))}] {\circled{2} Target state$^{}_{}$};
    \node [font=\scriptsize\scshape,color=white,text=black, at={(-3,-1.6))}] {\circled{3} Control $\mathbf{A}-30^{\circ}_{}$};
    \node [font=\scriptsize\scshape,color=white,text=black, at={(1.5,-1.6))}] {\circled{4} Control $\mathbf{B}+30^{\circ}_{}$};
    \node [font=\scriptsize\scshape,color=white,text=black, at={(6,-1.6))}] {\circled{5} Control $\mathbf{C}+90^{\circ}_{}$};
    \node [font=\scriptsize\scshape,color=white,text=black, at={(-0.5,-5.6))}] {\circled{6} Control $\mathbf{A}-30^{\circ}_{}$, $\mathbf{B}+30^{\circ}_{}$, $\mathbf{C}+30^{\circ}_{}$};
    \node [font=\scriptsize\scshape,color=white,text=black, at={(5,-5.6))}] {\circled{7} Control $\mathbf{C}+60^{\circ}_{}$};
\end{tikzpicture}

==> Chapter_2/euler_angles.tikz.tex <==
\def\radius{4}
\def\Alpha{25}
\def\Beta{20}
\def\Gamma{30}

\tdplotsetmaincoords{70}{150}

\tikzset{% Some styles. More could be done.
    axis/.style={thick, fill=black, -*, shorten >=-3pt},
    axis'/.style={-o, shorten >=-3pt},
    axis''/.style={-o, shorten >=-3pt},
    Axis/.style={thick, fill=black, -*, shorten >=-3pt}
}

\begin{tikzpicture}[tight background,auto]

\begin{scope}[scale=\radius, every path/.style={tdplot_rotated_coords}]

% Back half of the white circle.
\tdplotsetrotatedcoords{\Alpha}{0}{0}
\draw  [fill=MatlabBlue!50, opacity=0.5] 
    plot    [domain=90:270, samples=100] (cos \x, sin \x);

\tdplotsetrotatedcoords{\Alpha+90}{90}{0}
\draw [domain=90:90+\Beta, samples=100, dashed] plot (cos \x, sin \x);

% The light gray circle
\tdplotsetrotatedcoords{\Alpha}{\Beta}{\Gamma}
\draw  [fill=MatlabYellow!50, opacity=0.5] 
    plot    [domain=0:360, samples=100] (cos \x, sin \x);

% The front half of the white circle
\tdplotsetrotatedcoords{\Alpha}{0}{0}
\draw  [fill=MatlabBlue!50, opacity=0.5] 
    plot [domain=-90:90, samples=100] (cos \x, sin \x);

% The upper (unfilled) semi circles
\tdplotsetrotatedcoords{\Alpha}{90}{0}
\draw [domain=90:270, samples=100, dashed] plot (cos \x, sin \x);
\tdplotsetrotatedcoords{\Alpha+90}{90}{0}
\draw [domain=90+\Beta:270+\Beta, samples=100, dashed] plot (cos \x, sin \x);

% The X axis
\tdplotsetrotatedcoords{\Alpha}{\Beta}{\Gamma}
\draw[Axis] (0,0,0) -- (1,0,0) node [below left] {$X$};

% The x'' axis
\tdplotsetrotatedcoords{\Alpha}{\Beta}{0}
\draw[axis''] (0,0,0) -- (1,0,0) node [below left] {$x_{}^{\prime\prime}$};

% Axes x, y, z
\tdplotsetrotatedcoords{0}{0}{0}
\draw[axis] (0,0,0) -- (1,0,0) node [below left]  {$x$};
\draw[axis] (0,0,0) -- (0,1,0) node [below right] {$y$};
\draw[axis] (0,0,0) -- (0,0,1) node [above=0.1cm] {$z=z_{}^{\prime}$};

% Axis x'
\tdplotsetrotatedcoords{\Alpha}{0}{0}
\draw[axis'] (0,0,0) -- (1,0,0) node [below left] {$x_{}^{\prime}$};

% Axes Y
\tdplotsetrotatedcoords{\Alpha}{\Beta}{\Gamma}
\draw[Axis] (0,0,0) -- (0,1,0) node [right] {$Y$};

% Axes z' and Z
\draw[Axis] (0,0,0) -- (0,0,1) node [left=0.1cm] {$z_{}^{\prime\prime}=Z$};

% Axes y' and y''
\tdplotsetrotatedcoords{\Alpha}{\Beta}{0}
\draw[axis'] (0,0,0) -- (0,1,0) node [below right] {$y_{}^{\prime}=y_{}^{\prime\prime}$};

\tdplotsetrotatedcoords{0}{0}{0}
% Arrows
\tdplotsetrotatedcoords{0}{0}{0}
\tdplotdrawarc[-latex]{(0,0,0)}{0.8}{0}{\Alpha}{below left=-0.15cm}{$\alpha$}
\tdplotsetrotatedcoords{\Alpha+90}{90}{0}
\tdplotdrawarc[-latex]{(0,0,0)}{0.8}{-90}{-90+\Beta}{left}{$\beta$}
\tdplotsetrotatedcoords{\Alpha}{\Beta}{\Gamma}
\tdplotdrawarc[-latex]{(0,0,0)}{0.8}{-\Gamma}{0}{below}{$\gamma$}

\tdplotsetrotatedcoords{0}{0}{0}
\tdplotdrawarc[-latex]{(0,0,0)}{0.8}{90}{90+\Alpha}{above left=-0.15cm}{$\alpha$}
\tdplotsetrotatedcoords{\Alpha+90}{90}{0}
\tdplotdrawarc[-latex]{(0,0,0)}{0.8}{-180}{-180+\Beta}{above}{$\beta$}
\tdplotsetrotatedcoords{\Alpha}{\Beta}{\Gamma}
\tdplotdrawarc[-latex]{(0,0,0)}{0.8}{90-\Gamma}{90}{left}{$\gamma$}

\end{scope}

\end{tikzpicture}

==> Chapter_2/spherical_coordinates.tikz.tex <==
\tdplotsetmaincoords{60}{110}
%
\pgfmathsetmacro{\rvec}{0.8}
\pgfmathsetmacro{\thetavec}{40}
\pgfmathsetmacro{\phivec}{60}
%
\begin{tikzpicture}[scale=3,tight background,auto,tdplot_main_coords]
    \coordinate (O) at (0,0,0);
    \draw[thick,-latex] (0,0,0) -- (1,0,0) node[anchor=north east]{$x$};
    \draw[thick,-latex] (0,0,0) -- (0,1,0) node[anchor=north west]{$y$};
\draw[thick,-latex] (0,0,0) -- (0,0,1) node[anchor=south]{$z$};
    \tdplotsetcoord{P}{\rvec}{\thetavec}{\phivec}
    \draw[-*,color=MatlabRed,shorten >=-3pt] (O) -- (P) node[above right] {$r$};
    \draw[dashed, color=MatlabRed] (O) -- (Pxy);
    \draw[dashed, color=MatlabRed] (P) -- (Pxy);
    \tdplotdrawarc[color=MatlabRed]{(O)}{0.2}{0}{\phivec}{anchor=north}{$\varphi$}
    \tdplotsetthetaplanecoords{\phivec}
    \tdplotdrawarc[tdplot_rotated_coords,color=MatlabRed]{(0,0,0)}{0.5}{0}%
        {\thetavec}{anchor=south west}{\hspace{-0.3em}$\theta$}
    \draw[dashed,tdplot_rotated_coords] (\rvec,0,0) arc (0:90:\rvec);
\draw[dashed] (\rvec,0,0) arc (0:90:\rvec);
\node[align=left] at (0,2.2,0.6) 
    {\(x=r\sin\theta\cos\varphi\)\\ \(y=r\sin\theta\sin\varphi\)\\ \(z=r\cos\theta\)\vspace{2em}\\ \(r=\sqrt{x^2+y^2+z^2}\)\\ \(\varphi=\arctan\dfrac{y}{x}\)\\ \(\theta=\arccos\dfrac{z}{\sqrt{x^2+y^2+z^2}}\)\\ };
\end{tikzpicture}

==> Chapter_2/stern_gerlach.tikz.tex <==
\tikzset{
  beam action/.style={
    line width=\pgflinewidth+.2pt,draw opacity=.05,draw=#1,
  },
  beam recurs/.code 2 args={%
    \pgfmathtruncatemacro{\level}{#1-1}%
    \ifthenelse{\equal{\level}{0}}%
    {\tikzset{preaction={beam action=#2}}}%
    {\tikzset{preaction={beam action=#2,beam recurs={\level}{#2}}}}
  },
  beam/.style={preaction={beam recurs={33}{#1}},draw opacity=1,draw=#1},
}

\begin{tikzpicture}[tight background]
\begin{groupplot}[
		group style={
		group name=my plots,
		group size=1 by 1,
		y descriptions at=edge
		  left,
		x descriptions at=edge
		  bottom,
		horizontal sep=1.5em,
		vertical sep=2em,
		},
    width=0.75\columnwidth,
    compat=1.13,
    view={25}{-30},
    axis x line=middle,
    axis y line=middle,
    axis z line=middle,
    axis line style=-,
    xmin=0, xmax=100,
    ymin=-1, ymax=1,
    zmin=-1, zmax=1,
    xtick distance=5,
    minor x tick num = 0,
    scaled ticks=false,
    minor y tick num = 0,
    minor z tick num = 0,
    xticklabels={},
    xlabel={},
    ylabel={y},
    zlabel={z},
    xlabel style={anchor=north,xshift=0.2em,yshift=-0.2em,yslant=0.18,xscale=0.875},
    xtick align=center,
    ytick style={draw=none},
    ztick style={draw=none},
    x post scale=1.5,
    clip=false,
    hide axis,
]
\nextgroupplot[]
% SCREEN
           \addplot3+[ color=black, fill=MatlabYellow!10!white, opacity=1.0, solid, mark=none, ] 
           coordinates { (100, 1, 1) (100,-1, 1)
			 (100,-1,-1) (100, 1,-1) } --cycle;
     
     \path[line width=1.33pt,rounded corners=5mm,beam=MatlabBlue] (20,0,0) -- (80,0,0) -- (105,0,0.4375);
     \path[line width=1.33pt,rounded corners=5mm,beam=MatlabBlue] (20,0,0) -- (80,0,0) -- (105,0,-0.4375);
     
           \addplot3+[fill=MatlabYellow!10!white, opacity=1.0, draw=none, mark=none, ] 
           coordinates { (100, 0.75, 0.75) (100,0, 0.75)
			 (100,0,-0.75) (100, 0.75,-0.75) } --cycle;
     \node[below,yslant=-0.78,xscale=0.715] at (100,0,1) {Photographic plate};
     \path[preaction={fill=MatlabBlue},beam=MatlabBlue,rotate around={-50:(100,0,0.35)}] (100,0,0.35) circle(1.66pt and 0.66pt);
     \path[preaction={fill=MatlabBlue},beam=MatlabBlue,rotate around={-50:(100,0,0.35)}] (100,0,0.35) circle(1.66pt and 0.66pt);
     \path[preaction={fill=MatlabBlue},beam=MatlabBlue,rotate around={-50:(100,0,-0.35)}] (100,0,-0.35) circle(1.66pt and 0.66pt);
     \path[preaction={fill=MatlabBlue},beam=MatlabBlue,rotate around={-50:(100,0,-0.35)}] (100,0,-0.35) circle(1.66pt and 0.66pt);
     
     \node[MatlabBlue,right,yslant=-0.78,xscale=0.715] at (100,0.075,0.35) {$+\mu$};
     \node[MatlabBlue,right,yslant=-0.78,xscale=0.715] at (100,0.075,-0.35) {$-\mu$};

% MAGNET           
           \addplot3+[ color=black, fill=MatlabRed!40, opacity=0.5, solid, mark=none, ] 
           coordinates { ( 75,-0.25,-0.275) ( 30,-0.25,-0.275)
			 ( 30,-0.25, -0.75) ( 75,-0.25, -0.75)} --cycle;
           \addplot3+[ color=black, fill=MatlabRed!40, opacity=0.5, solid, mark=none, ] 
           coordinates { ( 75,-0.25,-0.275) ( 75, 0.00,-0.1) ( 75, 0.25,-0.275)
			 ( 75, 0.25, -0.75) ( 75,-0.25, -0.75)} --cycle;
           \addplot3+[ color=black, fill=MatlabRed!40, opacity=0.5, solid, mark=none, ] 
           coordinates { ( 75,-0.25,-0.275) ( 30,-0.25,-0.275)
			 ( 30, 0.00,-0.1) ( 75, 0.00,-0.1)} --cycle;
           \addplot3+[ color=black, fill=MatlabRed!40, opacity=0.5, solid, mark=none, ] 
           coordinates { ( 75, 0.00,-0.1) ( 30, 0.00,-0.1)
			 ( 30, 0.25,-0.275) ( 75, 0.25,-0.275)} --cycle;
           \addplot3+[ color=black, fill=MatlabRed!40, opacity=0.5, solid, mark=none, ] 
           coordinates { ( 75,-0.25, -0.75) ( 30,-0.25, -0.75)
			 ( 30, 0.25, -0.75) ( 75, 0.25, -0.75)} --cycle;
           \addplot3+[ color=black, fill=MatlabRed!40, opacity=0.5, solid, mark=none, ] 
           coordinates { ( 30,-0.25,-0.275) ( 30, 0.00,-0.1) ( 30, 0.25,-0.275)
			 ( 30, 0.25, -0.75) ( 30,-0.25, -0.75)} --cycle;
           \addplot3+[ color=black, fill=MatlabRed!40, opacity=0.5, solid, mark=none, ] 
           coordinates { ( 75, 0.25,-0.275) ( 30, 0.25,-0.275)
			 ( 30, 0.25, -0.75) ( 75, 0.25, -0.75)} --cycle;
     \node[black,above,yslant=0.17,xscale=0.875] at ( 52.5, 0.25, -0.75) {Magnet};
     \node[black,below,yslant=-0.78,xscale=0.715] at ( 30, 0, -0.125) {N};
     %\node[black,above,yslant=-0.78,xscale=0.715] at ( 30, 0, -0.75) {S};

           \addplot3+[ color=black, fill=MatlabBlue!40, opacity=0.5, solid, mark=none, ] 
           coordinates { ( 75,-0.25,0.1) ( 30,-0.25,0.1)
			 ( 30,-0.25, 0.75) ( 75,-0.25, 0.75)} --cycle;
           \addplot3+[ color=black, fill=MatlabBlue!40, opacity=0.5, solid, mark=none, ] 
           coordinates { ( 75,-0.25,0.1) ( 75, 0.25,0.1) 
			 ( 75, 0.25, 0.75) ( 75,-0.25, 0.75)} --cycle;
           \addplot3+[ color=black, fill=MatlabBlue!40, opacity=0.5, solid, mark=none, ] 
           coordinates { ( 75,-0.25,0.1) ( 30,-0.25,0.1)
			 ( 30, 0.25,0.1) ( 75, 0.25,0.1)} --cycle;
           \addplot3+[ color=black, fill=MatlabBlue!40, opacity=0.5, solid, mark=none, ] 
           coordinates { ( 75,-0.25, 0.75) ( 30,-0.25, 0.75)
			 ( 30, 0.25, 0.75) ( 75, 0.25, 0.75)} --cycle;
           \addplot3+[ color=black, fill=MatlabBlue!40, opacity=0.5, solid, mark=none, ] 
           coordinates { ( 30,-0.25,0.1) ( 30, 0.25,0.1)
			 ( 30, 0.25, 0.75) ( 30,-0.25, 0.75)} --cycle;
           \addplot3+[ color=black, fill=MatlabBlue!40, opacity=0.5, solid, mark=none, ] 
           coordinates { ( 75, 0.25,0.1) ( 30, 0.25,0.1)
			 ( 30, 0.25, 0.75) ( 75, 0.25, 0.75)} --cycle;
     \node[black,below,yslant=0.17,xscale=0.875] at ( 52.5, 0.25, 0.75) {Magnet};
     \node[black,above,yslant=-0.78,xscale=0.715] at ( 30, 0, 0.1) {S};
     %\node[black,below,yslant=-0.78,xscale=0.715] at ( 30, 0, 0.75) {N};
% SLITS
           \addplot3+[ color=black, fill=gray!50, opacity=0.75, solid, mark=none, ] 
           coordinates { (20, 0.33, 1.000) (20,-0.33, 1.000)
			 (20,-0.33, 0.075) (20, 0.33, 0.075) } --cycle;
           \addplot3+[ color=black, fill=gray!50, opacity=0.75, solid, mark=none, ] 
           coordinates { (20, 0.33,-0.075) (20,-0.33,-0.075)
			 (20,-0.33,-1.000) (20, 0.33,-1.000) } --cycle;

     \path[line width=1.33pt,rounded corners=5mm,beam=MatlabBlue] (15,0,0) -- (20,0,0);
     \path[line width=1.33pt,rounded corners=5mm,beam=MatlabBlue] (15,0,0) -- (20,0,0);
     
	   \addplot3+[ color=black, fill=gray!50, opacity=0.75, solid, mark=none, ] 
           coordinates { (15, 0.33, 1.000) (15,-0.33, 1.000)
			 (15,-0.33, 0.075) (15, 0.33, 0.075) } --cycle;
           \addplot3+[ color=black, fill=gray!50, opacity=0.75, solid, mark=none, ] 
           coordinates { (15, 0.33,-0.075) (15,-0.33,-0.075)
			 (15,-0.33,-1.000) (15, 0.33,-1.000) } --cycle;
     \node[below,yslant=-0.78,xscale=0.715] at (17.5,0,1.5) {Collimators};
     
     \path[line width=1.33pt,rounded corners=5mm,beam=MatlabBlue] (-2.5,0,0) -- (15,0,0);
     \path[line width=1.33pt,rounded corners=5mm,beam=MatlabBlue] (-2.5,0,0) -- (15,0,0);
     
           \addplot3+[ color=white, fill=white, opacity=1.0, solid, mark=none, ] 
           coordinates { (  0,-0.25,-0.25) (  0, 0,-0.25) 
			 (  0, 0, 0.25) (  0,-0.25, 0.25)} --cycle;
% OVEN
           \addplot3+[ color=black, fill=MatlabBlue!50, opacity=0.5, solid, mark=none, ] 
           coordinates { (  0,-0.25,-0.25) (-10,-0.25,-0.25)
			 (-10,-0.25, 0.25) (  0,-0.25, 0.25)} --cycle;
           \addplot3+[ color=black, fill=MatlabBlue!50, opacity=0.5, solid, mark=none, ] 
           coordinates { (  0,-0.25,-0.25) (  0, 0.25,-0.25) 
			 (  0, 0.25, 0.25) (  0,-0.25, 0.25)} --cycle;
           \addplot3+[ color=black, fill=MatlabBlue!50, opacity=0.5, solid, mark=none, ] 
           coordinates { (  0,-0.25,-0.25) (-10,-0.25,-0.25)
			 (-10, 0.25,-0.25) (  0, 0.25,-0.25)} --cycle;
           \addplot3+[ color=black, fill=MatlabBlue!50, opacity=0.5, solid, mark=none, ] 
           coordinates { (  0,-0.25, 0.25) (-10,-0.25, 0.25)
			 (-10, 0.25, 0.25) (  0, 0.25, 0.25)} --cycle;
           \addplot3+[ color=black, fill=MatlabBlue!50, opacity=0.5, solid, mark=none, ] 
           coordinates { (-10,-0.25,-0.25) (-10, 0.25,-0.25)
			 (-10, 0.25, 0.25) (-10,-0.25, 0.25)} --cycle;
           \addplot3+[ color=black, fill=MatlabBlue!50, opacity=0.5, solid, mark=none, ] 
           coordinates { (  0, 0.25,-0.25) (-10, 0.25,-0.25)
			 (-10, 0.25, 0.25) (  0, 0.25, 0.25)} --cycle;
     \node[below,yslant=0.17,xscale=0.875] at ( -5, 0.25, 0.25) {Oven};
\end{groupplot}

\end{tikzpicture}

==> Chapter_3/AdjointState_HC.tikz.tex <==
\begin{tikzpicture}[tight background]
\begin{groupplot}[
		group style={
		group name=my plots,
		group size=1 by 1,
		y descriptions at=edge
		  left,
		x descriptions at=edge
		  bottom,
		horizontal sep=2em,
		vertical sep=2em,
		},
    width=0.466\columnwidth,
    compat=1.13,
    axis x line=bottom,
    axis y line=left,
    axis line style=-,
    grid=both,
    xmin=0, xmax=50,
    ymin=0, ymax=1,
    xtick distance=5,
    ytick distance=0.2,
    minor y tick num = 3,
    minor x tick num = 4,
    scaled ticks=false,
    y tick label style={
        /pgf/number format/.cd,
            fixed,
            fixed zerofill,
            precision=1,
        /tikz/.cd
    },
    xlabel={time ({\normalfont{ms}})},
    groupplot ylabel={\footnotesize{{\scshape{Normalised Amplitudes}}}},
    tick align=outside,
    x post scale=2,
    clip=false,
]
\nextgroupplot[title style={at={(0.5,1.01875)},anchor=center,align=center},
	      title={$^{}_{}${\scshape Population at each spin}$^{}_{}$},]
    \coordinate (top) at (rel axis cs:0,1);
            \addplot+[o-{Latex},shorten <=-3pt,
               color=MatlabBlue,
               solid, thick,
               mark=none,
            ] table [x expr=\thisrowno{0}*1e3, y={Hfwd}] {\datadir/HC/Traj_HC.dat};
            \addplot+[o-{Latex},shorten <=-3pt,
               color=MatlabOrange,
               solid, thick,
               mark=none,
            ] table [x expr=\thisrowno{0}*1e3, y={Cfwd}] {\datadir/HC/Traj_HC.dat};
            \addplot+[{Latex}-o,shorten >=-3pt,
               color=MatlabBlue,
               dashed, thick,
               mark=none,
            ] table [x expr=\thisrowno{0}*1e3, y={Hbwd}] {\datadir/HC/Traj_HC.dat};
            \addplot+[{Latex}-o,shorten >=-3pt,
               color=MatlabOrange,
               dashed, thick,
               mark=none,
            ] table [x expr=\thisrowno{0}*1e3, y={Cbwd}] {\datadir/HC/Traj_HC.dat};
            
         \coordinate (bot) at (rel axis cs:1,0);
\end{groupplot}

\path[name path=p1] (top-|current bounding box.west)-- node[anchor=south,rotate=90] {} (bot-|current bounding box.west);
\path[name path=p2] (top|-current bounding box.north)-- coordinate(legendpos) (bot|-current bounding box.north);

\matrix[matrix of nodes, anchor=south, inner sep=0.2em, font=\sc\scriptsize, 
    column 1/.style={anchor=base east},
    column 2/.style={anchor=base east},
    column 3/.style={anchor=base west},
    column 4/.style={anchor=base east},
    column 5/.style={anchor=base west}] at (legendpos)
  {State trajectory, \(\big|\!\state(t)\big\rangle\): & [0.025\columnwidth]
   \draw[legendline={MatlabBlue}{1.00}] (-0.25,0.1) -- (0.25,0.1); & $_{}^{1}$H\hfill & [0.025\columnwidth]
   \draw[legendline={MatlabOrange}{1.00}] (-0.25,0.1) -- (0.25,0.1); & $_{}^{13}$C \\
   Adjoint state trajectory, \(\big\langle\!\Astate(t)\big|\): & [0.025\columnwidth]
   \draw[legenddash={MatlabBlue}{1.00}] (-0.25,0.1) -- (0.25,0.1); & $_{}^{1}$H & [0.025\columnwidth]
   \draw[legenddash={MatlabOrange}{1.00}] (-0.25,0.1) -- (0.25,0.1); & $_{}^{13}$C \\};

\end{tikzpicture}

==> Chapter_3/piecewise_const_xy.tikz.tex <==

\begin{tikzpicture}[tight background]
\begin{groupplot}[
		group style={
		group name=my plots,
		group size=1 by 1,
		y descriptions at=edge
		  left,
		x descriptions at=edge
		  bottom,
		horizontal sep=1.5em,
		vertical sep=2em,
		},
    width=0.85\columnwidth,
    compat=1.13,
    axis x line=middle,
    axis y line=middle,
    axis z line=middle,
    axis line style={latex}-{latex},
    x axis line style=-{latex},
    xmin=0, xmax=104.9,
    ymin=-1, ymax=1,
    zmin=-1, zmax=1,
    xtick distance=5,
    minor x tick num = 0,
    scaled ticks=false,
    ytick={-1},
    extra y ticks={1},
    every extra y tick/.style={yticklabels={$+x$},
	  yticklabel style={anchor=south west,xshift=-0.8em,yshift=-0.4em},},
    yticklabels={$-x$},
    yticklabel style={anchor=north east,xshift=0.6em,yshift=0.2em},
    ztick={-1},
    extra z ticks={1},
    every extra z tick/.style={zticklabels={$+y$},
	  zticklabel style={anchor=south,xshift=-0.1em,yshift=-0.2em},},
    zticklabels={$-y$},
    zticklabel style={anchor=north,xshift=0.1em,yshift=0.2em},
    minor y tick num = 0,
    minor z tick num = 0,
    xticklabels={},
    xlabel={time},
    xlabel style={anchor=north,xshift=0.2em,yshift=-0.2em,yslant=-0.18,xscale=0.875},
    xtick align=center,
    ytick style={draw=none},
    ztick style={draw=none},
    x post scale=1.5,
    clip=false,
]
\nextgroupplot[]
            \addplot3+[dashed, color=black!30,thin,mark=none,domain=0:2*pi,samples=100] (0,{sin(deg(x))},{cos(deg(x))});
            \draw [-latex,color=gray!85!MatlabBlue,font=\sc\scriptsize] (15,0.8,0.8) node[right,yslant=-0.18,xscale=0.875]{Transverse plane} to[out=170,in=25] (1,0.7,0.7);
            \addplot3+[
               color=black, fill=MatlabBlue!50, opacity=0.75,
               solid,
               mark=none,
            ] coordinates { (0,0.0000,0) (0,0.0000,0)
			    (5,0.0000,0) (5,0.3594,0)
			   (10,0.3594,0) (10,0.3102,0)
			   (15,0.3102,0) (15,0.0000,0)
			   (20,0.0000,0) (20,0.0000,0)
			   (25,0.0000,0) (25,0.0000,0)
			   (30,0.0000,0) (30,0.9195,0)
			   (35,0.9195,0) (35,0.0000,0)
			   (40,0.0000,0) (40,0.1705,0)
			   (45,0.1705,0) (45,0.0000,0)
			   (50,0.0000,0) (50,0.5025,0)
			   (55,0.5025,0) (55,0.0000,0)
			   (60,0.0000,0) (60,0.0119,0)
			   (65,0.0119,0) (65,0.3982,0)
			   (70,0.3982,0) (70,0.7818,0)
			   (75,0.7818,0) (75,0.9186,0)
			   (80,0.9186,0) (80,0.0944,0)
			   (85,0.0944,0) (85,0.0000,0)
			   (90,0.0000,0) (90,0.0000,0)
			   (95,0.0000,0) (95,0.0000,0)
			  (100,0.0000,0) (100,0.0000,0)};
            \addplot3+[
               color=black, fill=MatlabYellow!50, opacity=0.75,
               solid,
               mark=none,
            ] coordinates { (0,0, 0.0000) (0,0, 0.0000)
			    (5,0, 0.0000) (5,0,-0.9363)
			   (10,0,-0.9363) (10,0,-0.4462)
			   (15,0,-0.4462) (15,0,-0.9077)
			   (20,0,-0.9077) (20,0,-0.8057)
			   (25,0,-0.8057) (25,0, 0.0000)
			   (30,0, 0.0000) (30,0, 0.0000)
			   (35,0, 0.0000) (35,0,-0.3658)
			   (40,0,-0.3658) (40,0, 0.0000)
			   (45,0, 0.0000) (45,0,-0.9311)
			   (50,0,-0.9311) (50,0,-0.1225)
			   (55,0,-0.1225) (55,0,-0.2369)
			   (60,0,-0.2369) (60,0, 0.0000)
			   (65,0, 0.0000) (65,0, 0.0000)
			   (70,0, 0.0000) (70,0,-0.6263)
			   (75,0,-0.6263) (75,0,-0.0205)
			   (80,0,-0.0205) (80,0,-0.1088)
			   (85,0,-0.1088) (85,0, 0.0000)
			   (90,0, 0.0000) (90,0, 0.0000)
			   (95,0, 0.0000) (95,0, 0.0000)
			  (100,0, 0.0000) (100,0, 0.0000)};
            \addplot3+[
               color=black, fill=MatlabYellow!50, opacity=0.75,
               solid,
               mark=none,
            ] coordinates { (0,0,0.0000) (0,0,0.4121)
			    (5,0,0.4121) (5,0,0.0000)
			   (10,0,0.0000) (10,0,0.0000)
			   (15,0,0.0000) (15,0,0.0000)
			   (20,0,0.0000) (20,0,0.0000)
			   (25,0,0.0000) (25,0,0.6469)
			   (30,0,0.6469) (30,0,0.3897)
			   (35,0,0.3897) (35,0,0.0000)
			   (40,0,0.0000) (40,0,0.9004)
			   (45,0,0.9004) (45,0,0.0000)
			   (50,0,0.0000) (50,0,0.0000)
			   (55,0,0.0000) (55,0,0.0000)
			   (60,0,0.0000) (60,0,0.5310)
			   (65,0,0.5310) (65,0,0.5904)
			   (70,0,0.5904) (70,0,0.0000)
			   (75,0,0.0000) (75,0,0.0000)
			   (80,0,0.0000) (80,0,0.0000)
			   (85,0,0.0000) (85,0,0.2926)
			   (90,0,0.2926) (90,0,0.4187)
			   (95,0,0.4187) (95,0,0.5094)
			  (100,0,0.5094) (100,0,0.0000)};
            \addplot3+[
               color=black, fill=MatlabBlue!50, opacity=0.75,
               solid,
               mark=none,
            ] coordinates { (0, 0.0000,0) (0,-0.4479,0)
			    (5,-0.4479,0) (5, 0.0000,0)
			   (10, 0.0000,0) (10, 0.0000,0)
			   (15, 0.0000,0) (15,-0.6748,0)
			   (20,-0.6748,0) (20,-0.7620,0)
			   (25,-0.7620,0) (25,-0.0033,0)
			   (30,-0.0033,0) (30, 0.0000,0)
			   (35, 0.0000,0) (35,-0.3192,0)
			   (40,-0.3192,0) (40, 0.0000,0)
			   (45, 0.0000,0) (45,-0.5524,0)
			   (50,-0.5524,0) (50, 0.0000,0)
			   (55, 0.0000,0) (55,-0.4898,0)
			   (60,-0.4898,0) (60, 0.0000,0)
			   (65, 0.0000,0) (65, 0.0000,0)
			   (70, 0.0000,0) (70, 0.0000,0)
			   (75, 0.0000,0) (75, 0.0000,0)
			   (80, 0.0000,0) (80, 0.0000,0)
			   (85, 0.0000,0) (85,-0.7228,0)
			   (90,-0.7228,0) (90,-0.7014,0)
			   (95,-0.7014,0) (95,-0.4850,0)
			  (100,-0.4850,0) (100, 0.0000,0)};
     \node[above,color=gray!85!MatlabBlue,font=\sc\scriptsize,yslant=-0.18,xscale=0.875] at (2.5,0,0) {1};
     \node[above,color=gray!85!MatlabBlue,font=\sc\scriptsize,yslant=-0.18,xscale=0.875] at (27.5,0,0) {6};
     \node[above,color=gray!85!MatlabBlue,font=\sc\scriptsize,yslant=-0.18,xscale=0.875] at (32.5,0,0) {7};
     \node[above,color=gray!85!MatlabBlue,font=\sc\scriptsize,yslant=-0.18,xscale=0.875] at (42.5,0,0) {9};
     \node[above,color=gray!85!MatlabBlue,font=\sc\scriptsize,yslant=-0.18,xscale=0.875] at (62.5,0,0) {13};
     \node[above,color=gray!85!MatlabBlue,font=\sc\scriptsize,yslant=-0.18,xscale=0.875] at (67.5,0,0) {14};
     \node[above,color=gray!85!MatlabBlue,font=\sc\scriptsize,yslant=-0.18,xscale=0.875] at (87.5,0,0) {18};
     \node[above,color=gray!85!MatlabBlue,font=\sc\scriptsize,yslant=-0.18,xscale=0.875] at (92.5,0,0) {19};
     \node[above,color=gray!85!MatlabBlue,font=\sc\scriptsize,yslant=-0.18,xscale=0.875] at (97.5,0,0) {20};
     \node[above,color=gray!85!MatlabBlue,font=\sc\scriptsize,yslant=-0.18,xscale=0.875] at (47.5,0,-0.9311) {\(\Delta t\)};
     \draw [above,color=gray!85!MatlabBlue,thin, ->] (42.5,0,-0.82) to (45,0,-0.82);
     \draw [above,color=gray!85!MatlabBlue,thin, ->] (52.5,0,-0.82) to (50,0,-0.82);
\end{groupplot}

\end{tikzpicture}

==> Chapter_3/rosenbrock_convergence.tikz.tex <==
\begin{tikzpicture}[tight background]
\begin{groupplot}[
		group style={
		group name=my plots,
		group size=2 by 2,
		horizontal sep=2em,
		vertical sep=2em,
		},
    width=0.5\columnwidth,
    domain = -1.7:1.7,
    y domain = -0.7:3,
    point meta max=12.5,
    point meta min=-0.75757575,
    view={0}{90},
colormap={CM}{
samples of colormap=(32 of viridis)},
colormap access=piecewise constant,
hide axis,
]
\nextgroupplot[title style={at={(0.5,1.02)},anchor=center,align=center},
	      title={\plotlabel{a} $^{}_{}${\scshape Gradient Descent}$^{}_{}$},]
    \addplot3+[surf,shader=interp,mark=none,]{((1-x)^2 + 100*(y-x^2)^2)/100};
    \addplot+[color=white,mark=x] table {\datadir/Rosenbrock/rosenbrock_grad_descent.dat};
    \addplot3+[mark options={MatlabOrange!50,solid, fill=MatlabOrange},mark=triangle*] coordinates {(8.6538226e-01,7.3399446e-01,0.0)};

\nextgroupplot[title style={at={(0.5,1.02)},anchor=center,align=center},
	      title={\plotlabel{b} $^{}_{}${\scshape Symmetric rank-1 update}$^{}_{}$},]
    \addplot3+[surf,shader=interp,mark=none,]{((1-x)^2 + 100*(y-x^2)^2)/100};
    \addplot+[color=white,mark=x] table {\datadir/Rosenbrock/rosenbrock_sr1.dat};
    \addplot3+[mark options={MatlabOrange!50,solid, fill=MatlabOrange},mark=triangle*] coordinates {(8.6538226e-01,7.3399446e-01,0.0)};

\nextgroupplot[title style={at={(0.5,1.02)},anchor=center,align=center},
	      title={\plotlabel{c} $^{}_{}${\scshape BFGS rank-2 update}$^{}_{}$},]
    \addplot3+[surf,shader=interp,mark=none,]{((1-x)^2 + 100*(y-x^2)^2)/100};
    \addplot+[color=white,mark=x] table {\datadir/Rosenbrock/rosenbrock_bfgs.dat};
    \addplot3+[mark options={MatlabOrange!50,solid, fill=MatlabOrange},mark=triangle*] coordinates {(8.6538226e-01,7.3399446e-01,0.0)};

\nextgroupplot[title style={at={(0.5,1.02)},anchor=center,align=center},
	      title={\plotlabel{d} $^{}_{}${\scshape Newton-Raphson}$^{}_{}$},]
    \addplot3+[surf,shader=interp,mark=none,]{((1-x)^2 + 100*(y-x^2)^2)/100};
    \addplot+[color=white,mark=x] table {\datadir/Rosenbrock/rosenbrock_newton.dat};
    \addplot3+[mark options={MatlabOrange!50,solid, fill=MatlabOrange},mark=triangle*] coordinates {(8.6538226e-01,7.3399446e-01,0.0)};
    
\end{groupplot}
\end{tikzpicture}

==> Chapter_3/stationary_points.tikz.tex <==
\begin{tikzpicture}[tight background]
\begin{groupplot}[
		group style={
		group name=my plots,
		group size=3 by 1,
		horizontal sep=1em,
		vertical sep=1em,
		},
    width=0.4\columnwidth,
    samples=25,
    domain=-4:4,
    colormap/blackwhite,
    mesh/interior colormap name={viridis},
    hide axis,
]
\nextgroupplot[title style={at={(0.5,1)},anchor=center,align=center},
	      title={\plotlabel{a} $^{}_{}${\scshape Minimum}$^{}_{}$},
    view = {10}{50},]
    \addplot3[surf,
        ]{x^2 +y^2};
    \addplot3+[mark options={MatlabOrange!50,solid, fill=MatlabOrange},mark=triangle*] coordinates {(0.0,0.0,0.0)};

\nextgroupplot[title style={at={(0.5,1)},anchor=center,align=center},
	      title={\plotlabel{b} $^{}_{}${\scshape Maximum}$^{}_{}$},
    view = {20}{40},]
    \addplot3[surf,
        ]{-x^2 -y^2};
    \addplot3+[mark options={MatlabOrange!50,solid, fill=MatlabOrange},mark=triangle*] coordinates {(0.0,0.0,0.0)};

\nextgroupplot[title style={at={(0.5,1)},anchor=center,align=center},
	      title={\plotlabel{c} $^{}_{}${\scshape Saddle}$^{}_{}$},
    view = {30}{30},]
    \addplot3[surf,
        ]{x^2 -y^2};
    \addplot3+[mark options={MatlabOrange!50,solid, fill=MatlabOrange},mark=triangle*] coordinates {(0.0,0.0,0.0)};
\end{groupplot}

\end{tikzpicture}

==> Chapter_5/Parallelism.tikz.tex <==
\makeatletter
\def\parsenode[#1]#2\pgf@nil{%
    \tikzset{label node/.style={#1}}
    \def\nodetext{#2}
}

\tikzset{
    add node at x/.style 2 args={
        name path global=plot line,
        /pgfplots/execute at end plot visualization/.append={
                \begingroup
                \@ifnextchar[{\parsenode}{\parsenode[]}#2\pgf@nil
            \path [name path global = position line #1-1]
                ({axis cs:#1,0}|-{rel axis cs:0,0}) --
                ({axis cs:#1,0}|-{rel axis cs:0,1});
            \path [xshift=1pt, name path global = position line #1-2]
                ({axis cs:#1,0}|-{rel axis cs:0,0}) --
                ({axis cs:#1,0}|-{rel axis cs:0,1});
            \path [
                name intersections={
                    of={plot line and position line #1-1},
                    name=left intersection
                },
                name intersections={
                    of={plot line and position line #1-2},
                    name=right intersection
                },
                label node/.append style={pos=1}
            ] (left intersection-1) -- (right intersection-1)
            node [label node]{\nodetext};
            \endgroup
        }
    },
    add node at y/.style 2 args={
        name path global=plot line,
        /pgfplots/execute at end plot visualization/.append={
                \begingroup
                \@ifnextchar[{\parsenode}{\parsenode[]}#2\pgf@nil
            \path [name path global = position line #1-1]
                ({axis cs:0,#1}-|{rel axis cs:0,0}) --
                ({axis cs:0,#1}-|{rel axis cs:1,1});
            \path [yshift=1pt, name path global = position line #1-2]
                ({axis cs:0,#1}-|{rel axis cs:0,0}) --
                ({axis cs:0,#1}-|{rel axis cs:1,1});
            \path [
                name intersections={
                    of={plot line and position line #1-1},
                    name=left intersection
                },
                name intersections={
                    of={plot line and position line #1-2},
                    name=right intersection
                },
                label node/.append style={pos=1}
            ] (left intersection-1) -- (right intersection-1)
            node [label node] {\nodetext};
            \endgroup
        }
    }
}
\makeatother

\begin{tikzpicture}[tight background]
\begin{groupplot}[
		group style={
		group name=my plots,
		group size=1 by 1,
%
		x descriptions at=edge
		  bottom,
		y descriptions at=edge
		  left,
		horizontal sep=1em,
		vertical sep=0,
		},
    width=0.666\columnwidth,
    compat=1.13,
    ymin=1, ymax=9,
    axis x line=bottom,
    axis y line=left,
    axis line style=-,
    ytick distance=1,
    minor y tick num = 3,
    ylabel=Relative Speed-up,
    xmin=0, xmax=1,
    xtick distance=0.1,
    minor x tick num = 3,
    xlabel=Processor Cores / N,
    grid=both,
    y tick label style={
        /pgf/number format/.cd,
            fixed,
            fixed zerofill,
            precision=1,
        /tikz/.cd
    },
    x tick label style={
        /pgf/number format/.cd,
            fixed,
            fixed zerofill,
            precision=1,
        /tikz/.cd
    },
    max space between ticks=20,
    y post scale=1.125,
]
\nextgroupplot[title style={at={(0.5,1.05)},anchor=center,align=center},
	      title={$^{}_{}${\scshape Parallelisation}$^{}_{}$},]
               \coordinate (top) at (rel axis cs:0,1);
            \addplot+[smooth,
               samples=256,
               domain=0:1,
               color=black!75,
               mark=none,
               add node at x={0.25+0.042}{[color=black!75, font=\bf\scriptsize\sc, fill=white, inner xsep=2pt, inner ysep=0pt, opacity=1, text opacity=1, sloped]{100\% parallel}},
            ] {1/((1-1.0)+(1/(24*x))*1.0)};
	      
            \addplot+[smooth,
               samples=256,
               domain=0:1,
               color=black!75,
               dashed,
               mark=none,
               add node at x={0.4+0.042}{[color=black!75, font=\bf\scriptsize\sc, fill=white, inner xsep=2pt, inner ysep=0pt, opacity=1, text opacity=1, sloped]{ 90\% parallel}},
            ] {1/((1-0.9)+(1/(24*x))*0.9)};
            
            \addplot+[smooth,
               samples=256,
               domain=0:1,
               color=black!75,
               dashed,
               mark=none,
               add node at x={0.45+0.042}{[color=black!75, font=\bf\scriptsize\sc, fill=white, inner xsep=2pt, inner ysep=0pt, opacity=1, text opacity=1, sloped]{ 80\% parallel}},
            ] {1/((1-0.8)+(1/(24*x))*0.8)};
            
            \addplot+[smooth,
               samples=256,
               domain=0:1,
               color=black!75,
               dashed,
               mark=none,
               add node at x={0.475+0.042}{[color=black!75, font=\bf\scriptsize\sc, fill=white, inner xsep=2pt, inner ysep=0pt, opacity=1, text opacity=1, sloped]{ 70\% parallel}},
            ] {1/((1-0.7)+(1/(24*x))*0.7)};
            
            \addplot+[smooth,
               samples=256,
               domain=0:1,
               color=black!75,
               dashed,
               mark=none,
               add node at x={0.4875+0.042}{[color=black!75, font=\bf\scriptsize\sc, fill=white, inner xsep=2pt, inner ysep=0pt, opacity=1, text opacity=1, sloped]{ 60\% parallel}},
            ] {1/((1-0.6)+(1/(24*x))*0.6)};
            
            \addplot+[smooth,
               samples=256,
               domain=0:1,
               color=black!75,
               dashed,
               mark=none,
               add node at x={0.49375+0.042}{[color=black!75, font=\bf\scriptsize\sc, fill=white, inner xsep=2pt, inner ysep=0pt, opacity=1, text opacity=1, sloped]{ 50\% parallel}},
            ] {1/((1-0.5)+(1/(24*x))*0.5)};
            
            \addplot+[smooth,
               samples=256,
               domain=0:1,
               color=black!75,
               dashed,
               mark=none,
               add node at x={0.49375+0.042}{[color=black!75, font=\bf\scriptsize\sc, fill=white, inner xsep=2pt, inner ysep=0pt, opacity=1, text opacity=1, sloped]{ 40\% parallel}},
            ] {1/((1-0.4)+(1/(24*x))*0.4)};
            
            \addplot+[smooth,
               samples=256,
               domain=0:1,
               color=black!75,
               dashed,
               mark=none,
            ] {1/((1-0.3)+(1/(24*x))*0.3)};
            
            \addplot+[smooth,
               samples=256,
               domain=0:1,
               color=black!75,
               dashed,
               mark=none,
            ] {1/((1-0.2)+(1/(24*x))*0.2)};
            
            \addplot+[smooth,
               samples=256,
               domain=0:1,
               color=black!75,
               dashed,
               mark=none,
            ] {1/((1-0.1)+(1/(24*x))*0.1)};
            
            \addplot+[smooth,
               samples=256,
               domain=0:1,
               color=black!75,
               dashed,
               mark=none,
            ] {1/((1-0.0)+(1/(24*x))*0.0)};
            
            
            \addplot+[
               color=MatlabOrange,
               solid, thick,
               mark=o,
            ] table [x expr={\thisrowno{0}/24}, y expr={\thisrowno{1}}] {\datadir/grape_parallelism_HCF/ParComp.dat};
            \addplot+[
               color=MatlabBlue,
               solid, thick,
               mark=o,
            ] table [x expr={\thisrowno{0}/24}, y expr={\thisrowno{2}}] {\datadir/grape_parallelism_HCF/ParComp.dat};

         \coordinate (bot) at (rel axis cs:1,0);
\end{groupplot}

\path[name path=p1] (top-|current bounding box.west)-- node[anchor=south,rotate=90] {} (bot-|current bounding box.west);
\path[name path=p2] (top|-current bounding box.north)-- coordinate(legendpos) (bot|-current bounding box.north);

\matrix[matrix of nodes, anchor=south, inner sep=0.2em, font=\sc\scriptsize] at (legendpos)
  {\draw[legendline={MatlabBlue}{1.00}] (-0.25,0.1) -- (0.25,0.1); & Gradient calculation & [0.1\columnwidth]
   \draw[legendline={MatlabOrange}{1.00}] (-0.25,0.1) -- (0.25,0.1); & Hessian calculation \\};

\end{tikzpicture}

==> Chapter_6/Spillout_norm-cubed_pen.tikz.tex <==
\begin{tikzpicture}[tight background]
 \begin{axis}[
    width=0.666\columnwidth,
    xmin=-4.1, xmax=4.1,
    ymin=0, ymax=8.1,
    xtick distance=1, 
    ytick distance=1,
    minor x tick num = 3,
    minor y tick num = 3,
    grid=both,
    xlabel=Amplitude,
    ylabel=Penalty,
    x axis line style={latex-latex},
    y axis line style={-latex},
    ]
    
\addplot[smooth,MatlabBlue,mark=none,thick,samples=20,domain=1:3.1] 
	{((x-1)^3}
	node[color=MatlabBlue!50!black, anchor=west, pos=0.75] 
	{$\mathcal{K}$};
	
\addplot[smooth,MatlabBlue,mark=none,thick,samples=20,domain=-1:-3.1] 
	{((-x-1)^3}
	node[color=MatlabBlue!75!black, font=\bf\scriptsize\sc, sloped, anchor=north, pos=0.28] 
	{Fidelity};
	
\addplot[smooth,MatlabOrange,mark=none,thick,samples=20,domain=1:3.1] 
	{3*((x-1)^2)}
	node[color=MatlabOrange!50!black, anchor=west, pos=0.25] 
	{$\frac{d\mathcal{K}}{dc}$};
	
\addplot[smooth,MatlabOrange,mark=none,thick,samples=20,domain=-1:-3.1] 
	{3*((-x-1)^2)}
	node[color=MatlabOrange!75!black, font=\bf\scriptsize\sc, sloped, anchor=south, pos=0.28] 
	{Gradient};
	
\addplot[smooth,MatlabYellow,mark=none,thick,samples=20,domain=1:3.1] 
	{6*((x-1))}
	node[color=MatlabYellow!50!black, anchor=east, pos=0.25] 
	{$\frac{d^2\mathcal{K}}{d{c}^2}$};
	
\addplot[smooth,MatlabYellow,mark=none,thick,samples=20,domain=-1:-4.1] 
	{6*((-x-1))}
	node[color=MatlabYellow!75!black, font=\bf\scriptsize\sc, sloped, anchor=south, pos=0.28] 
	{Hessian};
	
\end{axis}
\end{tikzpicture}


==> Chapter_6/Spillout_norm-squared_pen.tikz.tex <==
\begin{tikzpicture}[tight background]
 \begin{axis}[
    width=0.666\columnwidth,
    xmin=-4.1, xmax=4.1,
    ymin=0, ymax=8.1,
    xtick distance=1, 
    ytick distance=1,
    minor x tick num = 3,
    minor y tick num = 3,
    grid=both,
    xlabel=Amplitude,
    ylabel=Penalty,
    x axis line style={latex-latex},
    y axis line style={-latex},
    ]
    
\addplot[smooth,MatlabBlue,mark=none,thick,samples=20,domain=1:4.1] 
	{((x-1)^2}
	node[color=MatlabBlue!50!black, anchor=east, pos=0.75] 
	{$\mathcal{K}$};
	
\addplot[smooth,MatlabBlue,mark=none,thick,samples=20,domain=-1:-4.1] 
	{((-x-1)^2}
	node[color=MatlabBlue!75!black, font=\bf\scriptsize\sc, sloped, anchor=south, pos=0.75] 
	{Fidelity};
	
\addplot[smooth,MatlabOrange,mark=none,thick,samples=2,domain=1:4.1] 
	{2*((x-1))}
	node[color=MatlabOrange!50!black, anchor=east, pos=0.65] 
	{$\frac{d\mathcal{K}}{dc}$};
	
\addplot[smooth,MatlabOrange,mark=none,thick,samples=2,domain=-1:-4.1] 
	{2*((-x-1))}
	node[color=MatlabOrange!75!black, font=\bf\scriptsize\sc, sloped, anchor=north, pos=0.75] 
	{Gradient};
	
\addplot[smooth,MatlabYellow,mark=none,thick,samples=2] 
	{2}
	node[color=MatlabYellow!75!black, font=\bf\scriptsize\sc, sloped, anchor=north, pos=0.2] 
	{Hessian}
	node[color=MatlabYellow!50!black, sloped, anchor=south, pos=0.6] 
	{$\frac{d^2\mathcal{K}}{d{c}^2}$};

\end{axis}
\end{tikzpicture}


==> Chapter_6/norm-squared_pen.tikz.tex <==
\begin{tikzpicture}[tight background]
 \begin{axis}[
    width=0.666\columnwidth,
    xmin=-4.1, xmax=4.1,
    ymin=0, ymax=8.1,
    xtick distance=1, 
    ytick distance=1,
    minor x tick num = 3,
    minor y tick num = 3,
    grid=both,
    xlabel=Amplitude,
    ylabel=Penalty,
    x axis line style={latex-latex},
    y axis line style={-latex},
    ]

\addplot[smooth,MatlabBlue,mark=none,thick,samples=20,domain=-4.1:4.1] 
	{x^2}
	node[color=MatlabBlue!50!black, anchor=east, pos=0.7] 
	{$\mathcal{K}$}
	node[color=MatlabBlue!75!black, font=\bf\scriptsize\sc, sloped, anchor=south, pos=0.3] 
	{Fidelity};
	
\addplot[smooth,MatlabOrange,mark=none,thick,samples=2,domain=0:4.1] 
	{2*x}
	node[color=MatlabOrange!50!black, anchor=east, pos=0.5] 
	{$\frac{d\mathcal{K}}{dc}$};
	
\addplot[smooth,MatlabOrange,mark=none,thick,samples=2,domain=0:-4.1] 
	{-2*x}
	node[color=MatlabOrange!75!black, font=\bf\scriptsize\sc, sloped, anchor=north, pos=0.6] 
	{Gradient};
	
\addplot[smooth,MatlabYellow,mark=none,thick,samples=2] 
	{2}
	node[color=MatlabYellow!75!black, font=\bf\scriptsize\sc, sloped, anchor=north, pos=0.2] 
	{Hessian}
	node[color=MatlabYellow!50!black, sloped, anchor=south, pos=0.55] 
	{$\frac{d^2\mathcal{K}}{d{c}^2}$};
	
	
\end{axis}
\end{tikzpicture}


==> Chapter_6/robustness_plot.tikz.tex <==
\begin{tikzpicture}[tight background]
\begin{groupplot}[
		group style={
		group name=my plots,
		group size=1 by 1,
		y descriptions at=edge
		  left,
		x descriptions at=edge
		  bottom,
		horizontal sep=0em,
		vertical sep=0em,
		},
    width=0.5\columnwidth,
    matrix rows=75,
    matrix cols=75,
    colormap/magma,
    axis on top,
    axis x line=bottom,
    axis y line=left,
    axis line style=-,
    xtick distance=25,
    ytick distance=25,
    xmin=-74.5, xmax=74.5,
    ymin=0.5, ymax=149.5,
    ylabel={Pulse Power},
    xlabel={Resonance Offset},
    y unit=Hz,
    x unit=Hz,
    unit markings=slash space,
    tick align=outside,
    ylabel near ticks,
    xlabel near ticks,
    point meta min=0,
    point meta max=0.707106781186548,
]
\nextgroupplot[
        matrix plot,point meta=explicit,
    ]
        \addplot+ table [
                    x expr={2*(\thisrowno{0}-38)},
                    y expr={2*(\thisrowno{1}-0.5)},
                    meta expr={\thisrowno{2}}] {\datafile};
    \coordinate (top) at (rel axis cs:0,1.05);

    \coordinate (bot) at (rel axis cs:1,0);
\end{groupplot}
% Node position middle above groupplot
\path (top|-current bounding box.north)--
                    coordinate(legendposabove)
                    (bot|-current bounding box.north);
\begin{axis}[%
  hide axis,
  scale only axis,
  width=0.5\columnwidth,
  at={(legendposabove.south)},
  yshift=1em,
  anchor=south,
  xmin=0, xmax=1,
  ymin=0, ymax=1,
  point meta min=0,
  point meta max=0.707106781186548,
  colormap/magma,                     % Colormap preset
  colorbar horizontal,                  % Active colorbar
  colorbar sampled,                     % Steps in colorbar
  colorbar style={
    xlabel={Fidelity, $2\Fid_1^{}$ / $\sqrt{2}$},
    height=.05\linewidth,
    separate axis lines,
    samples=256,                        % Number of steps
    xticklabel pos=upper,
    axis x line=top,
    axis y line=left,
    axis line style=-,
    xtick distance={2*0.0707106781186548},
    xticklabels={,
        $\leq\!0\phantom{\leq}$,$0.2\vphantom{\leq}$,$0.4\vphantom{\leq}$,$0.6\vphantom{\leq}$,$0.8\vphantom{\leq}$,$1.0\vphantom{\leq}$
    },
    xticklabel style={yshift=-0.25em},
    tick align=outside,
  },

]
  \addplot [draw=none] coordinates {(0,0)};
\end{axis}
\end{tikzpicture}

==> Chapter_6/waveform_plot.tikz.tex <==
\begin{tikzpicture}[tight background]
\begin{groupplot}[
		group style={
		group name=my plots,
		group size=2 by 1,
		y descriptions at=edge
		  left,
		x descriptions at=edge
		  bottom,
		horizontal sep=1.5em,
		},
    width=0.466\columnwidth,
    compat=1.13,
    axis x line=bottom,
    axis y line=left,
    axis line style=-,
    grid=both,
    xmin=0, xmax=112.5,
    ymin=-1, ymax=1,
    xtick distance=20,
    minor y tick num = 4,
    minor x tick num = 9,
    scaled ticks=false,
    yticklabel style={/pgf/number format/.cd,print sign},
    yticklabel={\ifdim\tick pt=0pt$0$\else\axisdefaultticklabel\fi},
    xlabel={time ({\normalfont{ms}})},
    groupplot ylabel={\footnotesize{{\scshape{Amplitude}}}},
    tick align=outside,
    axis x line=bottom,
    y post scale=0.5,
]
            
\nextgroupplot[title style={at={(0.5,1.03)},anchor=center,align=center},
	      title={\plotlabel{a} $^{}_{}${\scshape Pulse Sequence on }\(\HamHH_x^{}\)$^{}_{}$},]
            \addplot+[const plot,
               color=MatlabBlue, fill=MatlabBlue, fill opacity=0.25,
	       very thin,
               solid,
               mark=none,
            ] table [x expr=\thisrowno{0}*1e3, y={Lx}] {\wffile} \closedcycle;
            
\nextgroupplot[title style={at={(0.5,1.03)},anchor=center,align=center},
	      title={\plotlabel{b} $^{}_{}${\scshape Pulse Sequence on }\(\HamHH_y^{}\)$^{}_{}$},]
            \addplot+[const plot,
               color=MatlabOrange, fill=MatlabOrange, fill opacity=0.25,
	       very thin,
               solid,
               mark=none,
            ] table [x expr=\thisrowno{0}*1e3, y={Ly}] {\wffile} \closedcycle;
\end{groupplot}
\end{tikzpicture}
